Coco-Nut: Corpus of Japanese Utterance and Voice Characteristics Description for Prompt-based Control

In text-to-speech, controlling voice characteristics is important in achieving various-purpose speech synthesis. Considering the success of text-conditioned generation, such as text-to-image, free-form text instruction should be useful for intuitive and complicated control of voice characteristics. A sufficiently large corpus of high-quality and diverse voice samples with corresponding free-form descriptions can advance such control research. However, neither an open corpus nor a scalable method is currently available. To this end, we develop Coco-Nut, a new corpus including diverse Japanese utterances, along with text transcriptions and free-form voice characteristics descriptions. Our methodology to construct this corpus consists of 1) automatic collection of voice-related audio data from the Internet, 2) quality assurance, and 3) manual annotation using crowdsourcing. Additionally, we benchmark our corpus on the prompt embedding model trained by contrastive speech-text learning.

==> table/retrieved_pair_example.tex <==

\begin{table*}[t]
\centering 
\caption{Retrieved pair examples. ``Score'' means the average of subjective evaluated appropriateness. Text of each retrieved candidate means one characteristics prompt of retrieved candidate. Each text has been translated to English.}
\footnotesize
% \begin{tabular}{p{0.24\linewidth} p{0.05\linewidth}|p{0.24\linewidth} p{0.05\linewidth} p{0.24\linewidth} p{0.05\linewidth}}
\begin{tabular}{
p{0.26\linewidth} p{0.03\linewidth}|
p{0.26\linewidth} p{0.03\linewidth}
p{0.26\linewidth} p{0.03\linewidth}}
 Retrieval text & Score & 1st candidate & Score & 2-5th candidate & Score \\
 \hline
 A young woman in her twenties is speaking slowly with a sweet, clinging voice. & 8.40 &
 A young woman is speaking in a cloyingly sweet tone. & 8.15 &
 An elderly male is speaking slowly with a muffled voice. & 1.10 \\
 \hline
 A middle-aged cheerful man is speaking in a clear voice, addressing in a questioning manner. & 7.75 & 
 A man in his forties is speaking in a high-pitched voice, explaining something. & 5.00 & 
 A young man is speaking in a high-pitched voice, as if he is excited. & 2.35 \\
 \hline
 A young woman in her twenties is speaking with a cheerful voice. & 8.10 & 
 A young man is speaking in a gentle voice, whispering softly. & 1.05 &
 A man in his fifties. He has a casual tone and is speaking while occasionally pondering. & 1.70
\end{tabular}
\label{tab:retrieved-pair-examples}
\end{table*}



